A universal emulator for planar Ising lattices

We introduce the notion of an Ising emulator for two-dimensional Ising models: a broad class of flat, unit-edge-length lattices can be represented as site- or bond-diluted supercells of a single host lattice, for which the Feynman--Vdovichenko/Kac--Ward solution is fixed once and for all. We construct explicit square and triangular emulators and show that a single transition matrix, supplemented by lattice-specific binary masks, gives all the thermodynamic quantities of interest for both ferro- and antiferromagnetic couplings. We apply the framework to all eleven Archimedean lattices, to all twenty 2-uniform lattices -- whose thermodynamics is obtained here for the first time -- and to several pentagonal lattices, and show that the same construction extends directly to fractal and disordered Ising models, with no modification to the underlying machinery.

==> atlas_macros.tex <==
%% atlas_macros.tex — atlascard environment and supporting commands
%% Extracted from OneLatticeToRuleThemAll.tex; isings mapped to spblue.

% Colour alias: atlascard uses \isings; sp_template provides spblue.
\colorlet{isings}{black}

\providecommand{\NA}{---}
\providecommand{\sameasfm}{=}

%% ── Internal helpers ────────────────────────────────────────────────────────
\newcommand{\atlascardgrouphead}[1]{%
  {\scriptsize\bfseries\color{isings}#1}%
}

\newcommand{\atlasrulecolor}{gray!60}
\newcommand{\atlasruleweight}{0.5pt}
\newcommand{\atlasdividerweight}{0.45pt}

\newcommand{\atlascardminirule}{%
  {\color{\atlasrulecolor}\rule{\linewidth}{\atlasruleweight}}%
}

%% ── Number formatting for thermodynamic quantities ──────────────────────────
% \nfmt{decimal-places}{value-or-\NA}: rounds numeric values; passes \NA as-is.
\RequirePackage{siunitx}
\RequirePackage{xfp}
\newcommand{\nfmt}[2]{%
  \def\nfmtval{#2}\def\nfmtna{\NA}\def\nfmtnone{none}\def\nfmteq{\sameasfm}%
  \ifx\nfmtval\nfmtna\NA\else
  \ifx\nfmtval\nfmtnone\NA\else
  \ifx\nfmtval\nfmteq\sameasfm\else
    \num[round-mode=places,round-precision=#1,group-digits=false]{#2}%
  \fi\fi\fi
}
% \sfmt: 3 dp, drop trailing zeros so exact/near-zero values display as 0.
\newcommand{\sfmt}[1]{%
  \def\sfmtval{#1}\def\sfmtna{\NA}\def\sfmtnone{none}\def\sfmteq{\sameasfm}%
  \ifx\sfmtval\sfmtna\NA\else
  \ifx\sfmtval\sfmtnone\NA\else
  \ifx\sfmtval\sfmteq\sameasfm\else
    \num[round-mode=places,round-precision=3,round-pad=false,group-digits=false]{#1}%
  \fi\fi\fi
}

%% ── Structural metadata block ───────────────────────────────────────────────
\def\cardBondSite{}% default (empty until \cardtype or \carddatastruct sets it)
\newcommand{\cardtype}[1]{\def\cardBondSite{#1}}

% \atlasmetastructural{L}{|W|}{nv}{nl}{host}
\newcommand{\atlasmetastructural}[5]{%
\begingroup\scriptsize
\atlascardgrouphead{Structure}\par
\vskip 0.30em
{\renewcommand{\arraystretch}{1.18}%
\begin{tabular}{@{}r@{\;}c@{\;}l@{}}
$\mathrm{host}$ & $=$ & #5\\
$\mathrm{type}$ & $=$ & \cardBondSite\\
$L$             & $=$ & $#1$\\
$|\mathbb{W}|$  & $=$ & $#2$\\
$n_v$           & $=$ & $#3$\\
$n_l$           & $=$ & $#4$\\
\end{tabular}}%
\endgroup
}

%% ── Physics metadata blocks ─────────────────────────────────────────────────
\newlength{\atlasphysicslabelwidth}
\setlength{\atlasphysicslabelwidth}{1.15cm}
\newcommand{\atlasphysicslabel}[1]{\makebox[\atlasphysicslabelwidth][r]{$#1$}}

% Archimedean lattice (ferro + antiferro with 7 params)
% \atlasmetaphysicsarch{Tc}{ec}{A}{B}{TcAF}{ecAF}{s0AF}
\newcommand{\atlasmetaphysicsarch}[7]{%
\edef\cardTcD{\fpeval{round(-2/ln((exp(2/#1)-1)/(exp(2/#1)+1)), 5)}}%
\begingroup\scriptsize
\atlascardgrouphead{Thermodynamics}\par
\vskip 0.35em
{\scriptsize\itshape\color{isings} Ferromagnet}\par
\vskip 0.18em
{\renewcommand{\arraystretch}{1.18}%
\begin{tabular}{@{}r@{\;}c@{\;}l@{}}
$T_c$           & $=$ & $\nfmt{5}{#1}$\\
$\varepsilon_c$ & $=$ & $\nfmt{5}{#2}$\\
$A$             & $=$ & $\nfmt{5}{#3}$\\
$B$             & $=$ & $\nfmt{3}{#4}$\\
\end{tabular}}\par
\vskip 0.45em
\atlascardminirule\par
\vskip 0.45em
{\scriptsize\itshape\color{isings} Antiferromagnet}\par
\vskip 0.18em
{\renewcommand{\arraystretch}{1.18}%
\begin{tabular}{@{}r@{\;}c@{\;}l@{}}
$T_c^{\rm AF}$           & $=$ & $\nfmt{5}{#5}$\\
$\varepsilon_c^{\rm AF}$ & $=$ & $\nfmt{5}{#6}$\\
$s_0^{\rm AF}$           & $=$ & $\sfmt{#7}$\\
\end{tabular}}\par
\vskip 0.45em
\atlascardminirule\par
\vskip 0.45em
{\scriptsize\itshape\color{isings} Dual}\par
\vskip 0.18em
{\renewcommand{\arraystretch}{1.18}%
\begin{tabular}{@{}r@{\;}c@{\;}l@{}}
$T_c^{\rm D}$ & $=$ & $\cardTcD$\\
\end{tabular}}%
\endgroup
}

% Generic lattice (ferro + antiferro with 6 params)
% \atlasmetaphysicsgeneric{Tc}{ec}{A}{TcAF}{ecAF}{s0AF}
\newcommand{\atlasmetaphysicsgeneric}[6]{%
\edef\cardTcD{\fpeval{round(-2/ln((exp(2/#1)-1)/(exp(2/#1)+1)), 5)}}%
\begingroup\scriptsize
\atlascardgrouphead{Thermodynamics}\par
\vskip 0.35em
{\scriptsize\itshape\color{isings} Ferromagnet}\par
\vskip 0.18em
{\renewcommand{\arraystretch}{1.18}%
\begin{tabular}{@{}r@{\;}c@{\;}l@{}}
$T_c$           & $=$ & $\nfmt{5}{#1}$\\
$\varepsilon_c$ & $=$ & $\nfmt{5}{#2}$\\
$A$             & $=$ & $\nfmt{5}{#3}$\\
\end{tabular}}\par
\vskip 0.45em
\atlascardminirule\par
\vskip 0.45em
{\scriptsize\itshape\color{isings} Antiferromagnet}\par
\vskip 0.18em
{\renewcommand{\arraystretch}{1.18}%
\begin{tabular}{@{}r@{\;}c@{\;}l@{}}
$T_c^{\rm AF}$           & $=$ & $\nfmt{5}{#4}$\\
$\varepsilon_c^{\rm AF}$ & $=$ & $\nfmt{5}{#5}$\\
$s_0^{\rm AF}$           & $=$ & $\sfmt{#6}$\\
\end{tabular}}\par
\vskip 0.45em
\atlascardminirule\par
\vskip 0.45em
{\scriptsize\itshape\color{isings} Dual}\par
\vskip 0.18em
{\renewcommand{\arraystretch}{1.18}%
\begin{tabular}{@{}r@{\;}c@{\;}l@{}}
$T_c^{\rm D}$ & $=$ & $\cardTcD$\\
\end{tabular}}%
\endgroup
}

%% ── Convenience fillers ─────────────────────────────────────────────────────
\newcommand{\atlaspendingnote}[1]{%
\begin{minipage}[t]{\linewidth}\centering
\vspace{2.2em}
{\small\itshape #1}
\end{minipage}%
}

\newcommand{\atlasplotobject}[1]{%
\begin{minipage}[t]{\linewidth}\centering
\includegraphics[width=0.985\linewidth]{#1}
\end{minipage}
}

%% ── Path helpers for auto-label from image path ─────────────────────────────
% \atlascardlabelauto{dir/LABEL.png} -> \phantomsection\label{atlas:LABEL}
% Pure TeX string ops (no @ needed, no extra packages).
\newcommand{\atlascardlabelauto}[1]{\spstrippath#1/\relax}
\def\spstrippath#1/#2\relax{%
  \def\spstriptemp{#2}%
  \def\spstripempty{}%
  \ifx\spstriptemp\spstripempty
    \spstripext#1\relax
  \else
    \expandafter\spstrippath\spstriptemp\relax
  \fi
}
\def\spstripext#1.png\relax{\gdef\cardAutoName{#1}\phantomsection\label{atlas:#1}}

%% ── atlascard environment ───────────────────────────────────────────────────
% Usage:
%   \carddatastruct{L}{|W|}{nv}{nl}{type}
%   \cardphysicsarch{Tc}{ec}{A}{B}{TcAF}{ecAF}{s0AF}   % OR
%   \cardphysicsgeneric{Tc}{ec}{A}{TcAF}{ecAF}{s0AF}
%   \begin{atlascard}{Title}{image-path}{optional-header-note}
%     <right-column content: masks, plots, tables>
%   \end{atlascard}

\newlength{\atlascardslot}
\setlength{\atlascardslot}{0.49\textheight}

% Each card carries its own \captionof{figure} -- per explicit request, to
% remove any risk of a SciPost reviewer reading the family-level grouped
% caption as insufficient. Cost: fixed-height cards + a caption after each
% no longer fit two to a page (there isn't enough slack in \atlascardslot
% for both), so this reverts to roughly one card per page. The outer
% wrapper minipage keeps a card and its own caption from being split across
% a page break. \atlascardlabelauto still anchors atlas:<name> per card so
% \hyperref[atlas:...] links from the main-text summary tables resolve to
% the right card; \cardAutoName (set by the same macro) is reused for the
% per-card fig:atlas-<name> label.
\newenvironment{atlascard}[3]{%
\par\noindent
\begin{minipage}{\linewidth}% outer wrapper: keeps card + caption together
\begin{minipage}[t][\atlascardslot][t]{\linewidth}%
\atlascardlabelauto{#2}%
\gdef\cardTitle{#1}%
{\color{\atlasrulecolor}\rule{\linewidth}{\atlasruleweight}}\par
#3%
\xdef\cardCaptionL{\cardL}%
\xdef\cardCaptionBondSite{\cardBondSite}%
\nointerlineskip
\noindent
\begin{tabular}[t]{@{}p{0.204\textwidth}@{}!{\color{\atlasrulecolor}\vrule width \atlasdividerweight}@{\hspace{0.014\textwidth}}p{0.735\textwidth}@{}}
\begin{minipage}[t]{\linewidth}
{\centering\small\bfseries #1\par}
\vspace{0.45em}
{\centering\includegraphics[width=0.91\linewidth]{#2}\par}
\vskip 0.9em
{\raggedright\atlasmetastructural{\cardL}{\cardW}{\cardNv}{\cardNl}{\cardType}\par}
\vskip 0.6em
{\raggedright\atlascardminirule\par}
\vskip 0.6em
{\raggedright\cardphysicsblock\par}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}\vspace{0pt}%
}{%
\end{minipage}
\end{tabular}\par
\end{minipage}% close fixed-height card box
\vspace{0.4em}
\captionof{figure}{Atlas entry for the \cardTitle\ lattice: triangular-emulator \cardCaptionBondSite\ program at supercell size $L=\cardCaptionL$.}%
\label{fig:atlas-\cardAutoName}%
\end{minipage}\par
}

%% ── Card data helpers ───────────────────────────────────────────────────────
% \carddatastruct{L}{|W|}{nv}{nl}{bond|site}
\newcommand{\carddatastruct}[5]{%
  \def\cardL{#1}\def\cardW{#2}\def\cardNv{#3}\def\cardNl{#4}%
  \def\cardType{$\triangle$}%
  \def\cardBondSite{#5}%
}

% \cardphysicsarch{Tc}{ec}{A}{B}{TcAF}{ecAF}{s0AF}
\newcommand{\cardphysicsarch}[7]{%
  \def\cardphysicsblock{\atlasmetaphysicsarch{#1}{#2}{#3}{#4}{#5}{#6}{#7}}%
}

% \cardphysicsgeneric{Tc}{ec}{A}{TcAF}{ecAF}{s0AF}
\newcommand{\cardphysicsgeneric}[6]{%
  \def\cardphysicsblock{\atlasmetaphysicsgeneric{#1}{#2}{#3}{#4}{#5}{#6}}%
}

% \carddatageneric{L}{|W|}{Tc}{ec}{A}{AFtype}{ecAF}{s0AF}
% AFtype: "none" or \NA → frustrated, no AF transition; <number> → explicit TcAF
\newcommand{\carddatageneric}[8]{%
  \def\cardL{#1}%
  \def\cardW{#2}%
  \edef\cardNv{\the\numexpr #1*#1\relax}%
  \edef\cardNl{\the\numexpr 3*#1*#1\relax}%
  \def\cardType{$\triangle$}%
  \def\sp@afraw{#6}%
  \def\sp@afnone{none}%
  \def\sp@afNA{\NA}%
  \ifx\sp@afraw\sp@afnone
    \def\cardphysicsblock{%
      \atlasmetaphysicsgeneric{#3}{#4}{#5}{\NA}{#7}{#8}%
    }%
  \else
    \ifx\sp@afraw\sp@afNA
      \def\cardphysicsblock{%
        \atlasmetaphysicsgeneric{#3}{#4}{#5}{\NA}{#7}{#8}%
      }%
    \else
      \def\cardphysicsblock{%
        \atlasmetaphysicsgeneric{#3}{#4}{#5}{#6}{#7}{#8}%
      }%
    \fi
  \fi
}

% \cardcounts{nv}{nl}: actual number of lattice sites and bonds in the supercell
% (overrides the host-lattice defaults L^2 and 3L^2 set by \carddataarch)
\newcommand{\cardcounts}[2]{\edef\cardNv{#1}\edef\cardNl{#2}}

% \carddataarch{L}{|W|}{Tc}{ec}{A}{B}{AFtype}{ecAF}{s0AF}
% AFtype: "none"   → frustrated, no AF transition
%         \sameasfm → bipartite, TcAF = Tc
%         <number>  → frustrated with explicit TcAF
\newcommand{\carddataarch}[9]{%
  \def\cardL{#1}%
  \def\cardW{#2}%
  \edef\cardNv{\the\numexpr #1*#1\relax}%
  \edef\cardNl{\the\numexpr 3*#1*#1\relax}%
  \def\cardType{$\triangle$}%
  \def\sp@afraw{#7}%
  \def\sp@afnone{none}%
  \def\sp@afsameas{\sameasfm}%
  \ifx\sp@afraw\sp@afnone
    \def\cardphysicsblock{%
      \atlasmetaphysicsarch{#3}{#4}{#5}{#6}{\NA}{#8}{#9}%
    }%
  \else
    \ifx\sp@afraw\sp@afsameas
      \def\cardphysicsblock{%
        \atlasmetaphysicsarch{#3}{#4}{#5}{#6}{#3}{#8}{#9}%
      }%
    \else
      \def\cardphysicsblock{%
        \atlasmetaphysicsarch{#3}{#4}{#5}{#6}{#7}{#8}{#9}%
      }%
    \fi
  \fi
}

%% ── Grid layout for the restructured atlas (replaces per-lattice cards) ────
%% Each family is now: one grouped Fig. "lattices and supercell programs"
%% (one row per lattice: name/thumbnail + program mask(s)) and one grouped
%% Fig. "thermodynamic curves" (two four-panel plots per row). Numeric
%% thermodynamic data (Tc, epsilon_c, ...) is not repeated here -- it lives in
%% the main-text summary tables. \atlascardlabelauto keeps the same
%% atlas:<name> anchors so \hyperref[atlas:...] links from those tables still
%% resolve to the right row.

\newlength{\atlasgridrowheight}
\setlength{\atlasgridrowheight}{3.2cm}
\newlength{\atlasgridnamewidth}
\setlength{\atlasgridnamewidth}{0.22\textwidth}
\newlength{\atlasgridmaskswidth}
\setlength{\atlasgridmaskswidth}{0.74\textwidth}

% \atlasgridentry{name}{image}{annotation}{masks} -- one row: name, thumbnail,
% a one-line structural annotation ($L$, $n_v$, $n_l$) below it, then the
% program mask(s). Used uniformly across all three families; \atlascardlabelauto
% keeps the same atlas:<name> anchors so \hyperref[atlas:...] links from the
% main-text summary tables still resolve to the right row.
\newcommand{\atlasgridentry}[4]{%
\atlascardlabelauto{#2}%
\noindent
\begin{minipage}[c][\atlasgridrowheight][c]{\atlasgridnamewidth}\centering
{\small\bfseries #1}\\[0.35em]
\includegraphics[width=0.62\linewidth]{#2}\\[0.3em]
{\scriptsize\color{gray!70} #3}
\end{minipage}%
\begin{minipage}[c][\atlasgridrowheight][c]{\atlasgridmaskswidth}\centering #4\end{minipage}\par
\vspace{0.35em}
{\color{gray!40}\hrule}\par
\vspace{0.35em}
}

% \atlasthermocell{name}{pdf} -- one four-panel thermodynamic plot, meant to
% be used two per row (\hfill between them).
\newcommand{\atlasthermocell}[2]{%
\begin{minipage}[t]{0.47\textwidth}\centering
{\small\bfseries #1}\par\vspace{0.3em}
\includegraphics[width=\linewidth]{#2}
\end{minipage}%
}

